Pseudorandom (Function-Like) Quantum State Generators: New Definitions and Applications

Pseudorandom quantum states (PRS) are efficiently constructible states that are computationally indistinguishable from being Haar-random, and have recently found cryptographic applications. We explore new definitions, new properties and applications of pseudorandom states, and present the following contributions: 1. New Definitions: We study variants of pseudorandom function-like state (PRFS) generators, introduced by Ananth, Qian, and Yuen (CRYPTO'22), where the pseudorandomness property holds even when the generator can be queried adaptively or in superposition. We show feasibility of these variants assuming the existence of post-quantum one-way functions. 2. Classical Communication: We show that PRS generators with logarithmic output length imply commitment and encryption schemes with classical communication. Previous constructions of such schemes from PRS generators required quantum communication. 3. Simplified Proof: We give a simpler proof of the Brakerski--Shmueli (TCC'19) result that polynomially-many copies of uniform superposition states with random binary phases are indistinguishable from Haar-random states. 4. Necessity of Computational Assumptions: We also show that a secure PRS with output length logarithmic, or larger, in the key length necessarily requires computational assumptions.

==> approximatestategen.tex <==
% the following is for showing the output of purified unitary when the classical generation with abort is only approximate
statement: 
Let $G$ be a $(d, n)$-PRFS generator with classical generation with abort guarantee.
Fix $\lambda$ and let $\hat{G}$ denote the unitary part of $G_\lambda$ with $k, x$ hardcoded as input\footnote{See \Cref{sec:algorithms} for a definition of the unitary part of a generalized quantum circuit.}.
Then for all $k \in \{0,1\}^\lambda$, for all $x \in \{0,1\}^{d(\lambda)}$, there exists a negligible function $\eps(\cdot)$ such that
  \[
    \left \| \hat{G}\ket{0} - \left(\sqrt\eta \ket{\psi} \otimes \ket{anc} + \sqrt{1 - \eta}\ket\bot \otimes \ket{0}\right) \right \| \leq \eps(\lambda)
  \]
  where $\ket{0}$ denotes a suitable number of ancilla qubits, $\ket\psi$ and $\eta$ are those guaranteed by the classical generation with abort property (up to a global phase), and $\ket{anc}$ is some ancillary state that depends on $k,x$. 

The quantum circuit $G_\lambda$ take as input $\lambda + d(\lambda)$ qubits, and outputs $n(\lambda)$ qubits. Let $\hat{G}_\lambda$ denote its unitary part that acts on $n(\lambda) + b$ qubits where $b$ denotes the number of qubits that are traced out (which we denote by register $\reg{A}$).
Thus for all $k,x$ we have $G_\lambda(k,x) = \Tr_{\reg{A}} ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}})$ where $\ket{\Phi_{k,x}} = \hat{G}_\lambda \ket{k,x} \otimes \ket{0}^{\otimes a}$. By the state generation property, we have that $\TraceDist{ G_\lambda(k,x)}{ \ketbra{\psi_{k,x}}{\psi_{k,x}}} \leq \eps(\lambda)$ for some negligible function $\eps(\lambda)$. By \Cref{fact:td-to-fidelity}, this means that
\[
     \bra{\psi_{k,x}} G_\lambda(k,x) \ket{\psi_{k,x}} \geq \left ( 1 - \eps(\lambda) \right)^2~.
\]
Write $\ket{\Phi_{k,x}} = \alpha \ket{\psi_{k,x}} \otimes \ket{anc} + \beta \ket{\psi_\perp} \otimes \ket{anc'}$ for real numbers $\alpha,\beta$, some states $\ket{anc},\ket{anc'}$, and some state $\ket{\psi_\perp}$ that is orthogonal to $\ket{\psi_{k,x}}$. Then
\[
\bra{\psi_{k,x}} G_\lambda(k,x) \ket{\psi_{k,x}} = \Tr \left ( (\bra{\psi_{k,x}} \otimes I) \ketbra{\Phi_{k,x}}{\Phi_{k,x}} (\ket{\psi_{k,x}} \otimes I) \right) = \alpha^2 \, \Tr( \ketbra{anc}{anc}) = \alpha^2~.
\]
Therefore 
\[
    \left \| \ket{\Phi_{k,x}} - \ket{\psi_{k,x}} \otimes \ket{anc} \right \|^2 = 2 - 2 \alpha \leq 2 \eps(\lambda),
\]
and since $\sqrt{2 \eps(\lambda)}$ is a negligible function of $\lambda$, this concludes the proof of the Lemma.


\begin{lemma}[PRFS tester]
\label{lem:test}
Let $G$ be a PRFS generator with input length $d(\lambda)$ and output length $n(\lambda)$. Then there exists a QPT algorithm $\Test$ with boolean output and a negligible function $\eps(\lambda)$ such that for all $\lambda$, $k \in \{0,1\}^\lambda$, $x \in \{0,1\}^{d(\lambda)}$, and $n(\lambda)$-qubit density matrices $\rho$ we have that
\[
    \left | \Pr \Big [ \, \Test_\lambda(k,x,\rho) = 1 \, \Big ] - \bra{\psi_{k,x}} \, \rho \, \ket{\psi_{k,x}} \right| \leq \eps(\lambda)~.
\]
\end{lemma}
\begin{proof}
  Fix $\lambda$ and $k\in\{0,1\}^\lambda, x \in \{0,1\}^{d(\lambda)}$. It suffices to prove the Lemma in the case that $\rho$ is a pure state $\ketbra{\theta}{\theta}$; this is because if $\rho = \sum_j p_j \ketbra{\theta_j}{\theta_j}$ and if the acceptance probability of $\Test_\lambda(k,x,\ket{\theta_j})$ is $r_j$, then by linearity the acceptance probability of $\Test_\lambda(k,x,\rho)$ is going to be $\sum_j p_j r_j$, and therefore
  \[
    \left | \sum_j p_j r_j - \bra{\psi_{k,x}} \, \rho \, \ket{\psi_{k,x}} \right| \leq  \sum_j p_j \, \left | r_j - | \ip{\psi_{k,x}}{\theta_j} |^2 \right | \leq \sum_j p_j \eps(\lambda) \leq \eps(\lambda)
  \]
  as desired. So for the rest of this proof assume that $\rho = \ketbra{\theta}{\theta}$.
  
  Consider the unitary part $\hat{G}_\lambda$ of $G_\lambda$. It takes as input register $\reg{R} \reg{A}$ where $\reg{R}$ consists of $\lambda + d(\lambda)$ qubits. It outputs registers $\reg{R}' \reg{A}'$ where $\reg{R}'$ consists of $n(\lambda)$ qubits. From \Cref{lem:gen-unitary-part} we have that 
  \[
    \left \| \hat{G}_\lambda \ket{k,x}_{\reg{R}} \otimes \ket{0 \cdots 0}_{\reg{A}} - \ket{\psi_{k,x}}_{\reg{R}'} \otimes \ket{anc}_{\reg{A}'} \right \| \leq \eps(\lambda)
  \]
  for some negligible function $\eps(\lambda)$ and some state $\ket{anc}$. We now define the quantum circuit $\Test_\lambda$, which depends on $k,x$. Its unitary part $\widehat{\Test}_\lambda$ takes as input a $n(\lambda)$-qubit register $\reg{Q}$ and ancilla registers $\reg{R}, \reg{A}$. The circuit $\widehat{\Test}_\lambda$ behaves as follows:
  \begin{enumerate}
  	\item \label{alg:test-0} Initialize the register $\reg{R}$ in the state $\ket{k,x}$. 
  	\item \label{alg:test-1} Runs the unitary part $\hat{G}_\lambda$ on registers $\reg{R} \reg{A}$ to get registers $\reg{R}' \reg{A}'$~;
	\item \label{alg:test-2} Swaps the registers $\reg{Q}$ and $\reg{R}'$~;
	\item \label{alg:test-3} Applies the inverse $\hat{G}_\lambda^\dagger$ on registers $\reg{R}' \reg{A}'$ to get registers $\reg{R} \reg{A}$~;
	\item \label{alg:test-4} Measures the registers $\reg{R} \reg{A}$ and accept if and only if the outcome is $\ket{k,x} \otimes \ket{0 \cdots 0}$. 
\end{enumerate}
The quantum circuit $\Test_\lambda$ will run $\widehat{\Test}_\lambda$ with the ancilla register initialized to zeroes and at the end, traces out everything except for the decision bit. We define the quantum algorithm $\Test = \{ \Test_\lambda \}_\lambda$.

It is easy to see that $\Test$ is uniform and QPT (because $G$ is uniform and QPT). We now evaluate its acceptance probability on inputs of the form $(k,x,\ket{\theta})$. The state of $\widehat{\Test}_\lambda$ after Steps~\ref{alg:test-0} and~\ref{alg:test-1} is, by \Cref{lem:gen-unitary-part}, negligibly close, in Euclidean distance, to
\[
	\ket{\theta}_{\reg{Q}} \otimes \ket{\psi_{k,x}}_{\reg{R}'} \otimes \ket{anc}_{\reg{A}'}~.
\]
After Steps~\ref{alg:test-2} and~\ref{alg:test-3} the state is negligibly close to
\begin{equation}
\label{eq:test-final-state}
	\ket{\psi_{k,x}}_{\reg{Q}} \otimes \hat{G}^\dagger_\lambda \left ( \ket{\theta}_{\reg{R'}} \otimes \ket{anc}_{\reg{A}'} \right)~.
\end{equation}
The acceptance probability of $\widehat{\Test}_\lambda$ if the state were~\eqref{eq:test-final-state} would thus be
\begin{align*}
	\left |  \left ( \bra{k,x}_{\reg{R}} \otimes \bra{0 \cdots 0}_{\reg{A}} \right) \, \hat{G}^\dagger_\lambda \left ( \ket{\theta}_{\reg{R'}} \otimes \ket{anc}_{\reg{A}'} \right) \right |^2  = \left |  \bra{\Phi_{k,x}} \left ( \ket{\theta}_{\reg{R'}} \otimes \ket{anc}_{\reg{A}'} \right) \right |^2 
\end{align*}
%\\
%	& \qquad = \Tr \left ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}} \, \left( \ketbra{\theta}{\theta} \otimes \ketbra{anc}{anc} \right) \right) \\
%	&\qquad = \Tr \left ( \ketbra{\psi_{k,x}}{\psi_{k,x}} \, \ketbra{\theta}{\theta} \right) + \Tr \Big ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}} -  \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes \ketbra{anc}{anc} \Big)
%\end{align*}
where $\ket{\Phi_{k,x}} = \hat{G}_\lambda \ket{k,x,0 \cdots 0}$. Since $\ket{\Phi_{k,x}}$ is negligibly close to $\ket{\psi_{k,x}} \otimes \ket{anc}$ by \Cref{lem:gen-unitary-part}, we have that this quantity is negligibly close to 
\[
	\Big | \left( \bra{\psi_{k,x}} \otimes \bra{anc} \right) \left( \ket{\theta} \otimes \ket{anc} \right) \Big|^2 = \Big | \langle  \psi_{k,x} \, \mid \, \theta \rangle \Big|^2
\]
%	\Big \| \ketbra{\psi_{k,x}}{\psi_{k,x}} \, \ket{\theta} \Big \|^2~.
%\end{equation}
Thus we have shown that the acceptance probability of $\Test_\lambda$ on input $(k,x,\ket{\theta})$ is negligibly close to $|\langle \psi_{k,x} \mid \theta\rangle|^2$, which concludes the proof of the Lemma. 

%This is equivalent to the following quantity being negligible for all $\ket{\theta}$:
%\[
%	\Big | \, \bra{\theta} \otimes \bra{0 \cdots 0} \Big ( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I \Big) \ket{\theta} \otimes \ket{0 \cdots 0} \Big |~.
%\]
%This in turn implies that 
%\[
%	\left \| \Big( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I  \Big)  \ket{\theta} \otimes \ket{0 \cdots 0}  \right \|^2
%\]
%is negligible for all $\ket{\theta}$.

% we have the bound
%\begin{align*}
%\left | \Tr \Big ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}} -  \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes \ketbra{anc}{anc} \Big) \right | &\leq 2 \TraceDist{\ketbra{\Phi_{k,x}}{\Phi_{k,x}}}{\ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes \ketbra{anc}{anc}}\\
%& \leq 2 \left \| \ket{\Phi_{k,x}} - \ket{\psi_{k,x}} \otimes \ket{anc} \right \| \leq 2\eps(\lambda)
%\end{align*}
%where we used the fact that $|\Tr(A)| \leq \Tr(|A|)$. 



%  We compute $C$, swap out $\ket{\psi_{k, x}}$ with $\ket\theta$, uncompute $C$, and accept only if we get $\ket{0\cdots 0}$ back.
\end{proof}


Next we analyze a \emph{product} of $\Test$ algorithms run in parallel on different qubits of a (possibly entangled) state $\ket{\Phi}$. Before doing so, we show that we can express the behavior of a single invocation of the $\Test$ algorithm as a projection onto the input state. To do so, observe that by definition of the $\Test$ algorithm, the acceptance probability can be written as
\[
	\left \| P \, \widehat{\Test}_\lambda \, \ket{\theta}_{\reg{Q}} \otimes \ket{0 \cdots 0}_{\reg{R} \reg{A}} \right \|^2
\]
where $P$ is a projection that checks whether $\reg{R} \reg{A}$ is in the state $\ket{k,x,0\cdots 0}$. Since $\widehat{\Test}_\lambda$ is unitary and the Euclidean norm is unitarily invariant, this quantity is the same as 
\[
	\left \| \Pi \, \ket{\theta}_{\reg{Q}} \otimes \ket{0 \cdots 0}_{\reg{R} \reg{A}} \right \|^2
\]
where $\Pi = \widehat{\Test}_\lambda^\dagger \, P \, \widehat{\Test}_\lambda$ is a projection. We say that $\Pi$ is the projection corresponding to the $\Test(k,x,\cdot)$ algorithm accepting.

\Cref{lem:test} shows that the following quantity being negligible for all $\ket{\theta}$:
\[
	\Big | \, \bra{\theta} \otimes \bra{0 \cdots 0} \Big ( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I \Big) \ket{\theta} \otimes \ket{0 \cdots 0} \Big |~.
\]
This in turn implies that 
\begin{equation}
\label{eq:test-proj}
	\left \| \Big( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I  \Big)  \ket{\theta} \otimes \ket{0 \cdots 0}  \right \|^2
\end{equation}
is negligible for all $\ket{\theta}$.

\begin{lemma}[Product of PRFS testers]
\label{lem:test-product}
Let $G$ be a PRFS generator and let $\Test$ denote the corresponding tester algorithm given by \Cref{lem:test}. Fix $\lambda, t \in \N$. For all $k_1,\ldots,k_t \in \{0,1\}^\lambda$ and for all $x_1,\ldots,x_t \in \{0,1\}^{d(\lambda)}$, define the QPT algorithm $\Test^{\otimes t}$ that given an $t\cdot n(\lambda)$-qubit density matrix $\rho$ behaves as follows: for all $i=1,\ldots,t$, on the $i$'th block of $n(\lambda)$ qubits of $\rho$, run the algorithm $\Test_\lambda(k_i,x_i,\cdot)$. Output $1$ if and only if all $t$ invocations of $\Test$ output $1$. Then
\[
    \left | \Pr \Big [ \Test^{\otimes t} (k_1,x_1,\ldots,k_t,x_t,\rho) = 1 \Big] - \bra{\psi} \, \rho \, \ket{\psi} \right | \leq t^2 \cdot \eps(\lambda)
\]
for some negligible function $\eps(\lambda)$, where $\ket{\psi} = \ket{\psi_{k_1,x_1}} \otimes \cdots \otimes \ket{\psi_{k_t,x_t}}$.
\end{lemma}
\begin{proof}
  Fix $\lambda, t$, and $t \cdot n(\lambda)$-qubit state $\rho$. Like in \Cref{lem:test}, it suffices to prove the Lemma in the case that $\rho$ is a pure state $\ketbra{\Phi}{\Phi}$. Let $\reg{Q}_1,\ldots,\reg{Q}_t$ denote the $n(\lambda)$-qubit registers of $\ket{\Phi}$. Consider the $i$'th invocation of the $\Test$ algorithm, denoted by $\Test_i$, which acts on register $\reg{Q}_i$ and an ancilla register $\reg{A}_i$ (which implicitly includes the register $\reg{R}$ from \Cref{lem:test}). Let $\Pi_i$ denote the projector corresponding to $\Test_i(k_i,x_i,\cdot)$ accepting. From~\eqref{eq:test-proj} we have that for all $n(\lambda)$-qubit states $\ket{\varphi}$, 
  \[
    \left \| \Big( \Pi_i - \ketbra{\psi_{k_i,x_i}}{\psi_{k_i,x_i}} \otimes I \Big) \ket{\varphi}_{\reg{Q}_i} \otimes \ket{0 \cdots 0}_{\reg{A}_i} \right \| \leq \eps(\lambda)
  \]
  for some negligible function $\eps(\lambda)$. By a hybrid argument, for all $t \cdot n(\lambda)$-qubit states $\ket{\Phi}$, we have
  \[
    \left \| \, \left ( \bigotimes_i \Pi_i - \bigotimes_i \ketbra{\psi_{k_i,x_i}}{\psi_{k_i,x_i}} \otimes I \right) \ket{\Phi}_{\reg{Q}} \otimes \ket{0 \cdots 0}_{\reg{A}} \right \| \leq t \cdot \eps(\lambda)
  \]
  where $\reg{Q} = \reg{Q}_1 \cdots \reg{Q}_t$ and $\reg{A} = \reg{A}_1 \cdots \reg{A}_t$. 
  Note that the probability $\Test^{\otimes t}$ accepts on input $\ket{\Phi}$ is equal to $ \left \| \Big(\bigotimes_i \Pi_i \Big) \ket{\Phi} \otimes \ket{0 \cdots 0} \right \|^2$, whereas 
  \[
    \left \| (\bigotimes_i \ketbra{\psi_{k_i,x_i}}{\psi_{k_i,x_i}} \otimes I) \ket{\Phi} \otimes \ket{0 \cdots 0} \right \|^2 = \left | \langle \Phi \, \mid \, \psi_{k_1,x_1},\ldots,\psi_{k_t,x_t} \rangle \right |^2~.
  \]
  Using the fact that for all unit vectors $a,b$ the following inequality holds: $\Big | \| a\|^2 - \|b\|^2 \Big | \leq  2 \| a - b \|^2$, we obtain the statement of the Lemma.
\end{proof}



%%% starting here is the old Test lemma proof
It is easy to see that $\Test$ is uniform and QPT (because $G$ is uniform and QPT). We now evaluate its acceptance probability on inputs of the form $(k,x,\ket{\theta})$. The state of $\widehat{\Test}_\lambda$ after Steps~\ref{alg:test-0} and~\ref{alg:test-1} is, by \Cref{lem:gen-unitary-part}, negligibly close, in Euclidean distance, to
\[
	\ket{\theta}_{\reg{Q}} \otimes \ket{\psi_{k,x}}_{\reg{R}'} \otimes \ket{anc}_{\reg{A}'}~.
\]
After Steps~\ref{alg:test-2} and~\ref{alg:test-3} the state is negligibly close to
\begin{equation}
\label{eq:test-final-state}
	\ket{\psi_{k,x}}_{\reg{Q}} \otimes \hat{G}^\dagger_\lambda \left ( \ket{\theta}_{\reg{R'}} \otimes \ket{anc}_{\reg{A}'} \right)~.
\end{equation}
The acceptance probability of $\widehat{\Test}_\lambda$ if the state were~\eqref{eq:test-final-state} would thus be
\begin{align*}
	\left |  \left ( \bra{k,x}_{\reg{R}} \otimes \bra{0 \cdots 0}_{\reg{A}} \right) \, \hat{G}^\dagger_\lambda \left ( \ket{\theta}_{\reg{R'}} \otimes \ket{anc}_{\reg{A}'} \right) \right |^2  = \left |  \bra{\Phi_{k,x}} \left ( \ket{\theta}_{\reg{R'}} \otimes \ket{anc}_{\reg{A}'} \right) \right |^2 
\end{align*}
%\\
%	& \qquad = \Tr \left ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}} \, \left( \ketbra{\theta}{\theta} \otimes \ketbra{anc}{anc} \right) \right) \\
%	&\qquad = \Tr \left ( \ketbra{\psi_{k,x}}{\psi_{k,x}} \, \ketbra{\theta}{\theta} \right) + \Tr \Big ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}} -  \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes \ketbra{anc}{anc} \Big)
%\end{align*}
where $\ket{\Phi_{k,x}} = \hat{G}_\lambda \ket{k,x,0 \cdots 0}$. Since $\ket{\Phi_{k,x}}$ is negligibly close to $\ket{\psi_{k,x}} \otimes \ket{anc}$ by \Cref{lem:gen-unitary-part}, we have that this quantity is negligibly close to 
\[
	\Big | \left( \bra{\psi_{k,x}} \otimes \bra{anc} \right) \left( \ket{\theta} \otimes \ket{anc} \right) \Big|^2 = \Big | \langle  \psi_{k,x} \, \mid \, \theta \rangle \Big|^2
\]
%	\Big \| \ketbra{\psi_{k,x}}{\psi_{k,x}} \, \ket{\theta} \Big \|^2~.
%\end{equation}
Thus we have shown that the acceptance probability of $\Test_\lambda$ on input $(k,x,\ket{\theta})$ is negligibly close to $|\langle \psi_{k,x} \mid \theta\rangle|^2$, which concludes the proof of the Lemma. 

%This is equivalent to the following quantity being negligible for all $\ket{\theta}$:
%\[
%	\Big | \, \bra{\theta} \otimes \bra{0 \cdots 0} \Big ( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I \Big) \ket{\theta} \otimes \ket{0 \cdots 0} \Big |~.
%\]
%This in turn implies that 
%\[
%	\left \| \Big( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I  \Big)  \ket{\theta} \otimes \ket{0 \cdots 0}  \right \|^2
%\]
%is negligible for all $\ket{\theta}$.

% we have the bound
%\begin{align*}
%\left | \Tr \Big ( \ketbra{\Phi_{k,x}}{\Phi_{k,x}} -  \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes \ketbra{anc}{anc} \Big) \right | &\leq 2 \TraceDist{\ketbra{\Phi_{k,x}}{\Phi_{k,x}}}{\ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes \ketbra{anc}{anc}}\\
%& \leq 2 \left \| \ket{\Phi_{k,x}} - \ket{\psi_{k,x}} \otimes \ket{anc} \right \| \leq 2\eps(\lambda)
%\end{align*}
%where we used the fact that $|\Tr(A)| \leq \Tr(|A|)$. 



%  We compute $C$, swap out $\ket{\psi_{k, x}}$ with $\ket\theta$, uncompute $C$, and accept only if we get $\ket{0\cdots 0}$ back.


%%% finally, some misc stuff before proof of product
\Cref{lem:test} shows that the following quantity being negligible for all $\ket{\theta}$:
\[
	\Big | \, \bra{\theta} \otimes \bra{0 \cdots 0} \Big ( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I \Big) \ket{\theta} \otimes \ket{0 \cdots 0} \Big |~.
\]
This in turn implies that 
\begin{equation}
\label{eq:test-proj}
	\left \| \Big( \Pi - \ketbra{\psi_{k,x}}{\psi_{k,x}} \otimes I  \Big)  \ket{\theta} \otimes \ket{0 \cdots 0}  \right \|^2
\end{equation}
is negligible for all $\ket{\theta}$.

%%% and the proof for product
\begin{proof}
  Fix $\lambda, t$, and $t \cdot n(\lambda)$-qubit state $\rho$. Like in \Cref{lem:test}, it suffices to prove the Lemma in the case that $\rho$ is a pure state $\ketbra{\Phi}{\Phi}$. Let $\reg{Q}_1,\ldots,\reg{Q}_t$ denote the $n(\lambda)$-qubit registers of $\ket{\Phi}$. Consider the $i$'th invocation of the $\Test$ algorithm, denoted by $\Test_i$, which acts on register $\reg{Q}_i$ and an ancilla register $\reg{A}_i$ (which implicitly includes the register $\reg{R}$ from \Cref{lem:test}). Let $\Pi_i$ denote the projector corresponding to $\Test_i(k_i,x_i,\cdot)$ accepting. From~\eqref{eq:test-proj} we have that for all $n(\lambda)$-qubit states $\ket{\varphi}$, 
  \[
    \left \| \Big( \Pi_i - \ketbra{\psi_{k_i,x_i}}{\psi_{k_i,x_i}} \otimes I \Big) \ket{\varphi}_{\reg{Q}_i} \otimes \ket{0 \cdots 0}_{\reg{A}_i} \right \| \leq \eps(\lambda)
  \]
  for some negligible function $\eps(\lambda)$. By a hybrid argument, for all $t \cdot n(\lambda)$-qubit states $\ket{\Phi}$, we have
  \[
    \left \| \, \left ( \bigotimes_i \Pi_i - \bigotimes_i \ketbra{\psi_{k_i,x_i}}{\psi_{k_i,x_i}} \otimes I \right) \ket{\Phi}_{\reg{Q}} \otimes \ket{0 \cdots 0}_{\reg{A}} \right \| \leq t \cdot \eps(\lambda)
  \]
  where $\reg{Q} = \reg{Q}_1 \cdots \reg{Q}_t$ and $\reg{A} = \reg{A}_1 \cdots \reg{A}_t$. 
  Note that the probability $\Test^{\otimes t}$ accepts on input $\ket{\Phi}$ is equal to $ \left \| \Big(\bigotimes_i \Pi_i \Big) \ket{\Phi} \otimes \ket{0 \cdots 0} \right \|^2$, whereas 
  \[
    \left \| (\bigotimes_i \ketbra{\psi_{k_i,x_i}}{\psi_{k_i,x_i}} \otimes I) \ket{\Phi} \otimes \ket{0 \cdots 0} \right \|^2 = \left | \langle \Phi \, \mid \, \psi_{k_1,x_1},\ldots,\psi_{k_t,x_t} \rangle \right |^2~.
  \]
  Using the fact that for all unit vectors $a,b$ the following inequality holds: $\Big | \| a\|^2 - \|b\|^2 \Big | \leq  2 \| a - b \|^2$, we obtain the statement of the Lemma.
\end{proof}


==> bqp_neq_pp.tex <==
\begin{theorem}
  Let $G$ be a PRS generator with output length $n(\lambda) \geq (1 + \eps) \log \lambda$ for some constant $\eps > 0$.
  Then $BQP \neq PP$.
\end{theorem}
\begin{proof}
  We consider the same two cases as the proof for \Cref{lem:prs-inefficient-dist} except we replace the constant with $.9$.
  In case 1 where there does not exist a negligible function $\nu(\cdot)$ that satisfies
  \begin{equation}
    \label{eq:purity-test-pp}
    \Pr_k\left[\min_{\ket\theta}\TD(G_\lambda(k), \ketbra\theta\theta) \le \nu(\lambda)\right] \ge .9,
  \end{equation}
  we note that the $A$ could be generalized here and is efficient.
  Therefore, case 1 PRS cannot exist.
  
  We now consider case 2 where there exists a negligible function $\nu(\cdot)$ that satisfies \eqref{eq:purity-test-pp}.
  Similar as before we define the set $g$ and $\ket{\psi_k} = \arg\min_{\ket\theta}\TD(G_\lambda(k), \ketbra\theta\theta)$.
  
  Let $T = O(\lambda)$ where the exact constant will be chosen later.
  We construct the language $L$ to consist of all $(x, C)$ such that the probability of observing $x$ when measuring $G_\lambda(k)^{\otimes T}$ for a random $k \in \bit^\lambda$ under Clifford basis $C$ is more likely than that when measuring $T$ copies of random Haar state under the same basis $C$.
  This language is in $PP = PostBQP$ as we can prepare either with probability $1/2$ each, and look at what we have prepared post selecting on the event that we measured $x$ under basis $C$.
  \luowen{We might need to argue that the post selected event happens with at least exponentially small probability? William however did not argue this}
  
  We show how to use this language as an oracle to efficiently break computational indistinguishability, which means that the language cannot be in $BQP$ as otherwise we would have an efficient distinguisher between the two distributions.
  
  We first claim that the total variation distance of random Clifford basis measurements are noticeable as well.
  Let $\rho_\lambda, \sigma_\lambda$ denote the density matrices of the output of $G_\lambda()$ and $H_\lambda()$ respectively.
  For every $k \in g$, we define observable $O_k = \ketbra{\psi_k}{\psi_k}$.
  Note that when an unknown state $\rho$ comes from $G$, with probability at least $.9$ there exists an observable $O_k$ such that $\Tr(O_k\rho) \ge 1 - \nu(\lambda)$.
  On the other hand, it is easy to see by Haar measure concentration and union bound that $\Tr(O_k\rho) < \frac13$ for all $k \in g$, except with probability at most $2^\lambda \cdot e^{-2^n/3}$ which is negligible as $n \ge (1 + \eps) \log\lambda$. \luowen{TODO Need to copy the lemma over, and possibly the theorem from \cite{Huang2020}}
  Invoking \cite{Huang2020}, there is an algorithm that uses the measurement results to estimate the value of the observable $O$ for an unknown mixed state such that with probability $.9$, the estimated value is correct up to additive error $1/6$, if $T = O(\lambda)$.
  Therefore, with probability at least $.8$, the algorithm is able to distinguish $\rho_\lambda$ from $\sigma_\lambda$ by simply analyzing the measurement outcomes.
  The correctness of the algorithm implies that the total variation distance of the random measurements must be at least constant-far as well.
  
  Now we construct the distinguisher, which simply samples a random Clifford basis, measures the input in that basis, and output $G$ if the oracle thinks the measurement outcomes are more likely come from $G$, or Haar random otherwise.
  By the Bayes decision rule, this algorithm also distinguishes $\rho_\lambda$ from $\sigma_\lambda$ with probability at least $.8$, breaking the PRS security.
  This is a contradiction and therefore the language cannot be in $BQP$.
\end{proof}


==> more_elaborate_binary_phase.tex <==

Note that $\mu$, the distribution from which the states $\ket{\varphi_x}$ are sampled from, is \emph{isotropic} in the sense that it satisfies
\begin{equation}
\label{eq:isotropy}
    \E_{\ket{\varphi} \sim \mu} \ket{\varphi} = 0
\end{equation}
and
\begin{equation}
    \label{eq:sym-avg}
    \E_{\ket{\varphi} \sim \mu} \ketbra{\varphi}{\varphi} = 2^{-n} \, I
\end{equation}
where $I$ denotes the $2^n \times 2^n$ identity matrix. 
%Examples of isotropic distributions $\mu$ are: the Haar measure over $\C^d$, and in the case of $d = 1$, the uniform distribution over $\{\pm 1\}$.

\begin{lemma}
\label{lem:binaryphase}
Fix $t,d,n \in \N$. Let $\{ \ket{\varphi_x} \}_{x \in \{0,1\}^d}$ be a collection of i.i.d. states in $\C^{2^n}$ sampled from $\mu$, indexed by strings $x \in \{0,1\}^d$. 
Define
\[
\ket{\psi} = 2^{-n/2} \sum_{x \in \{0,1\}^d} \ket{x} \otimes \ket{\varphi_x}.
\]
Then
\begin{equation}
\label{eq:td1}
	\TD \Big (\,  \E  \ketbra{\psi}{\psi}^{\otimes t} \, , \, \E  \ketbra{\vartheta}{\vartheta}^{\otimes t} \, \Big ) \leq O(t/2^{n/2})
\end{equation}
where $\ket{\vartheta}$ is a Haar-random $(d+n)$-qubit state.
\end{lemma}

This Lemma is also the main result of~\cite{brakerski2020quantum}, except they obtain a better error for~\eqref{eq:td1} of $O(t^2/2^d)$. Our error bound is quadratically worse, but still suffices for the purpose of proving \Cref{thm:prfs-to-prs}. 

\begin{proof}
 Let $N = 2^n$ and $D = 2^d$. Let $\Pi_\sym = \Pi_\sym^{DN,t}$ be the projector onto the symmetric subspace of $(\C^{DN})^{\otimes t}$. We show~\eqref{eq:td1} via the following calculation. 
By \Cref{fact:avg-haar-random} we have that~\eqref{eq:td1} is equal to
\[
\TD \left ( \E  \ketbra{\psi}{\psi}^{\otimes t} , \frac{\Pi_\sym}{\Tr(\Pi_\sym)} \right ).
\]
We argue that $\ket{\psi}^{\otimes t}$ is close to $(\Pi_\distinct \otimes I) \ket{\psi}^{\otimes t}$, where $\Pi_\distinct$ is the projection onto the first $n$ qubits
\[
	\Pi_\distinct := \sum_{(x_1,\ldots,x_t) \in \distinct(d,t)} \ketbra{x_1,\ldots,x_t}{x_1,\ldots,x_t}
\]
where $\distinct(d,t)$ denote the set of all distinct tuples $(x_1,\ldots,x_t) \in (\{0,1\}^d)^t$. We now appeal to the principle of gentle measurement. Performing the binary measurement $\{ \Pi_\distinct, I - \Pi_\distinct \}$ on the state $\ket{\psi}^{\otimes t}$ is the same as measuring the state in the standard basis and accepting if the resultant tuple $(x_1,\ldots,x_t)$ consists of $t$ distinct $d$-bit strings. The probability that there is a collision is at most $O(t^2/D)$; therefore
\[
	\left \| \ket{\psi}^{\otimes t} - \Pi_\distinct \ket{\psi}^{\otimes t} \right \|^2 = \left \| (I - \Pi_\distinct) \ket{\psi}^{\otimes t} \right \|^2 \leq O(t^2/D)~.
\]
Therefore, since the trace distance between two pure states is at most a constant times their Euclidean distance, 
\begin{equation}
\label{eq:td1.5}
	\TD \left ( \ketbra{\psi}{\psi}^{\otimes t} , \Pi_\distinct \, \ketbra{\psi}{\psi}^{\otimes t} \, \Pi_\distinct \right) \leq O(t/D^{1/2})~.
\end{equation}
Thus, up to error $O(t/D^{1/2})$, we can approximate~\eqref{eq:td1} with 
\begin{equation}
\label{eq:td2}
	\TD \Big ( \E  \Pi_\distinct \ketbra{\psi}{\psi}^{\otimes t} \Pi_\distinct \, , \, \frac{\Pi_\sym}{\Tr(\Pi_\sym)} \Big )
\end{equation}
instead. 

Expanding out the definition of the first argument we get
\begin{equation}
\label{eq:td3}
	\E \Pi_\distinct \ketbra{\psi}{\psi}^{\otimes t} \Pi_\distinct = D^{-t}  \E \sum_{\substack{(x_1,\ldots,x_t) \in \distinct(d,t) \\ (y_1,\ldots,y_t)  \in \distinct(d,t)}}  \bigotimes_i  \ketbra{x_i}{y_i} \otimes \ketbra{\varphi_{x_i}}{\varphi_{y_i}}~.
\end{equation}
Bringing in the expectation, we get that the ``matrix coefficient'' corresponding to the block \\  $\ketbra{x_1,\ldots,x_t}{y_1,\ldots,y_t}$ is
\begin{equation}
\label{eq:ex1}
\E  \ketbra{\varphi_{x_1}}{\varphi_{y_1}} \otimes \cdots \otimes \ketbra{\varphi_{x_t}}{\varphi_{y_t}}~.
\end{equation}
Since $(x_1,\ldots,x_t)$ and $(y_1,\ldots,y_t)$ are tuples in $\distinct(d,t)$, it must be that for each $i \in [t]$, there exists at most one $j \in [t]$ such that $x_i = y_j$; in this case we say that $x_i$ and $y_j$ are \emph{paired}. If there is any $x_{i'}$ (or $y_{j'}$) that is unpaired, then the expectation~\eqref{eq:ex1} vanishes, because of property~\eqref{eq:isotropy} of the distribution $\mu$ (i.e. the expectation of an unpaired vector $\ket{\varphi_{x_{i'}}}$ is $0$).
%because $\alpha_{x_{i'}}$ (or $\alpha_{y_{j'}}$) is a uniformly random $\pm 1$ variable.

Thus the summation in~\eqref{eq:td3} can be simplified to being over all tuples $(x_1,\ldots,x_t) \in \distinct(d,t)$ and their \emph{permutations}, 
%and the expectation in~\eqref{eq:ex1} becomes $1$ (because all $x_i$'s are paired with exactly one $y_j$), 
so that~\eqref{eq:td3} can be written as
\begin{equation}
\label{eq:td4}
D^{-t}  \sum_{\substack{(x_1,\ldots,x_t) \in \distinct(d,t) \\ \sigma \in S_t}} \bigotimes_i  \ketbra{x_i}{x_{\sigma(i)}} \otimes \ketbra{\varphi_{x_i}}{\varphi_{x_{\sigma(i)}}}~.
\end{equation}
For a permutation $\sigma \in S_t$, let $P_\sigma$ denote the unitary acting on $(\C^{D})^{\otimes t} \otimes (\C^N)^{\otimes t}$ that permutes the $t$ tensor factors $\C^D \otimes \C^N$ according to $\sigma$. Define
\begin{align}
A &= N^t \, \sum_{(x_1,\ldots,x_t) \in \distinct(d,t)} \ketbra{x_1,\ldots,x_t}{x_1,\ldots,x_t} \otimes \E \ketbra{\varphi_{x_1},\ldots,\varphi_{x_t}}{\varphi_{x_1},\ldots,\varphi_{x_t}} \\
&= \sum_{(x_1,\ldots,x_t) \in \distinct(d,t)} \ketbra{x_1,\ldots,x_t}{x_1,\ldots,x_t} \otimes I^{\otimes t}
\end{align}
where the second line follows from~\eqref{eq:sym-avg} applied to each $\ketbra{\varphi_{x_i}}{\varphi_{x_i}}$. 
Then notice that~\eqref{eq:td4} is equal to
\begin{equation}
\label{eq:td5}
(DN)^{-t} \cdot A \cdot \left (\sum_{\sigma \in S_t} P_\sigma \right) = (DN)^{-t} \cdot \left (\sum_{\sigma \in S_t} P_\sigma \right) \cdot A~.
\end{equation}
In other words, $\sum_\sigma P_\sigma$ commutes with $A$. Using $\Pi_\sym = \frac{1}{t!} \sum_\sigma P_\sigma$, we thus get 
\begin{equation}
    \label{eq:binary-phase-5}
\E \Pi_\distinct \, \ketbra{\psi}{\psi}^{\otimes t} \, \Pi_\distinct = c  \Pi_\sym \, A \, \Pi_\sym
\end{equation}
where $c = (DN)^{-t} \cdot (t!)^{-1}$. We now argue that $c \Pi_\sym \, A \, \Pi_\sym$ is close to $c \Pi_\sym$:
\begin{equation}
    \label{eq:binary-phase-6}
 \left \|c \Pi_\sym -  c \Pi_\sym \, A \, \Pi_\sym \right \|_1 =  c  \, \Tr \left ( \Pi_\sym \,( I -  A) \, \Pi_\sym \right)
\end{equation}
where the equality follows from the fact that $\Pi_\sym \,( I -  A) \, \Pi_\sym$ is a positive operator (because $A$ is a positive operator whose operator norm is at most $1$). We calculate the difference $
 c \, \Tr(\Pi_\sym) - c \, \Tr(\Pi_\sym\, A \, \Pi_\sym)$. By \Cref{fact:sym-dim-approx}, we have that the first term $ c \, \Tr(\Pi_\sym)$ is at most $1 + O(t^2/DN)$. We bound the second term as follows:
\begin{align}
c \, \Tr(\Pi_\sym\, A \, \Pi_\sym) &= \Tr \left ( \E \Pi_\distinct \, \ketbra{\psi}{\psi}^{\otimes t} \, \Pi_\distinct \right ) \\
&= \E \left \|  \Pi_\distinct \, \ket{\psi}^{\otimes t} \right \|^2 \\
&\geq 1 - O(t^2/D)~.
\end{align}
Combining \Cref{eq:binary-phase-5,eq:binary-phase-6}, this implies that $\E \Pi_\distinct \, \ketbra{\psi}{\psi}^{\otimes t} \, \Pi_\distinct$ is $O(t^2/D)$-close in trace distance to the operator $c \Pi_\sym$, which (by \Cref{fact:sym-dim-approx} again) is $O(t^2/D)$-close to the density operator $\Pi_\sym/\Tr(\Pi_\sym)$. This shows that~\eqref{eq:td2} is at most $O(t^2/D)$. 

Combining our bounds on~\eqref{eq:td1.5} and~\eqref{eq:td2} via the triangle inequality, we get that
\[
	\TD \Big ( \E   \ketbra{\psi}{\psi}^{\otimes t} \, , \, \E  \ketbra{\vartheta}{\vartheta}^{\otimes t} \Big ) \leq O(t/D^{1/2})
\]
as desired.

==> old_stuff.tex <==

\begin{comment}
\hnote{This follow Lemma is not used anywhere in this paper, is it?}
\begin{lemma}
\label{lem:prs-prefix-prob}

Let $G$ be a $n(\lambda)$-PRS generator. Let $d(\lambda)$ be a function where $d(\lambda) \leq n(\lambda)$ and $d(\lambda) = O(\log \lambda)$. Then there exists a negligible function $\eps(\lambda)$ such that for all $\lambda$, for all $x \in \{0,1\}^{d(\lambda)}$, we have
\[
    \Pr_{k \leftarrow \{0,1\}^\lambda} \Big [ \Big | p_{k,x} - 2^{-d(\lambda)} \Big| \geq 2^{-d(\lambda)}/2 \Big] \leq \eps(\lambda)~.
\]
where $p_{k,x}$ is the probability that measuring the first $d(\lambda)$ qubits of $G_\lambda(k)$ yields the outcome $x$. 
\end{lemma}
\begin{proof}
For notational convenience we write $d = d(\lambda)$ and $n = n(\lambda)$. Suppose with nonnegligible probability $1/q(\lambda)$ over $k \leftarrow \{0,1\}^\lambda$, the probability $p_{k,x}$ deviated from $2^{-d}$ by more than $2^{-d}/2$ -- call such $k$'s \emph{bad}. We design a QPT algorithm $A$ to distinguish between $G$ and Haar-random states. The algorithm takes as input $\ket{\psi}^{\otimes t}$ where we set $t = 2^{2d + 3} \cdot \lambda$ (note that $t$ is a polynomial in $\secparam$ since $d = O(\log \lambda)$).  It measures the first $d$ qubits of each copy of $\ket{\psi}$ and counts the number of times $r$ it obtains the outcome $x$. If $|r/t - 2^{-d}| \geq 2^{-d}/4$, then the algorithm rejects; otherwise it accepts. For a fixed $k$, by a Chernoff-Hoeffding bound we have that
\[
    \Pr \Big [ |r/t - p_{k,x}| \geq \delta\Big ] \leq 2 \exp(-2 \delta^2 t )
\]
where the probability is over the randomness of the measurement outcomes. Suppose that $k$ is bad. Then letting $\delta = 2^{-d}/4$ the probability that the algorithm rejects is at least $1 - 2 \exp(-2^{-2d - 3} t)$. Thus averaged over the keys $k$, the rejection probability of $A$ on input $G_\lambda(k)^{\otimes t}$ is at least 
\[
    \frac{1}{q(\lambda)} (1 - 2 \exp(-2^{-2d -3 }t)) \geq \frac{1 - 2 e^{-\secparam}}{q(\lambda)}
\]
which is nonnegligible. On the other hand, the rejection probability of $A$ on input $\ket{\vartheta}^{\otimes t}$ is negligible when $\ket{\vartheta}$ is sampled from the Haar measure $\Haar_n$. 

\note{HY: this needs more explanation} This contradicts the pseudorandomness property of $G$.
\end{proof}
\end{comment}

\iffalse
\luowen{the following does not work. commented out.}
\section{Computationally indistinguishable quantum channels implies $BQP \neq PP$}
\begin{theorem}
  Assuming the existence of two quantum polynomial-time channels $G, H$, such that $\TD(G_\lambda(), H_\lambda()) = 1/\lambda^{O(1)}$, and $G_\lambda() \approx_c H_\lambda()$.
  Then $BQP \neq PP$.
\end{theorem}
\begin{proof}[Proof sketch]
  Let $\eps = \TD(G_\lambda(), H_\lambda())$.
  Let $T = O(1/\eps^2)$ where the exact constant will be chosen later.
  We construct the language $L_G$ to consist of all $(x, C)$ such that the probability of observing $x$ when measuring $G_\lambda^{\otimes T}$ under Clifford basis $C$ is at least that when measuring $H_\lambda^{\otimes T}$ under the same basis $C$.
  This language is in $PP = PostBQP$ as we can prepare either $G$ or $H$ with probability $1/2$ each, and look at what we have prepared post selecting on the event that we measured $x$ under basis $C$.
  \luowen{We might need to argue that the post selected event happens with at least exponentially small probability?}
  
  We show how to use this language as an oracle to efficiently break computational indistinguishability, which means that the language cannot be in $BQP$ as otherwise we would have an efficient distinguisher between the two distributions.
  
  We first claim that the total variation distance of random Clifford basis measurements are noticeable as well.
  Let $\rho_\lambda, \sigma_\lambda$ denote the density matrices of the output of $G_\lambda()$ and $H_\lambda()$ respectively.
  There is a normalized observable $O$ that implements the optimal distinguishing measurement, such that $|\Tr(O\rho_\lambda) - \Tr(O\sigma_\lambda)| \ge \eps$.
  \luowen{The next step has a bug! In particular, HKP's sample size depends on the Hilbert--Schmidt norm of $O$, and in this case it might be exponentially larger than its operator norm.}
  Invoking \cite{Huang2020}, there is an algorithm that uses the measurement results to estimate the value of the observable $O$ for an unknown mixed state such that with probability $.99$, the estimated value is correct up to additive error $\eps/3$, if $T = O(1/\eps^2)$.
  Therefore, with probability $.99$, the algorithm is able to distinguish $\rho_\lambda$ from $\sigma_\lambda$ by simply analyzing the measurement outcomes.
  The correctness of the algorithm implies that the total variation distance of the random measurements must be $.99$-far as well.
  
  Now we construct the distinguisher, which simply samples a random Clifford basis, measures the input in that basis, and output $G$ if the oracle thinks the measurement outcomes are more likely come from $G$, or $H$ otherwise.
  By the Bayes decision rule, this algorithm also distinguishes $\rho_\lambda$ from $\sigma_\lambda$ with probability $.99$, breaking the computational indistinguishability.
  This is a contradiction and therefore the language cannot be in $BQP$.
\end{proof}
\fi



%%%%%%%%%%%%%%%%%%%%%% STATE GENERATION FOR PRS -> PRFS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \paragraph{State generation.} From the state generation property of $G$, there exists $\ket{\psi_k}$ such that $\TraceDist{G_\secparam(k)}{\ketbra{\psi_{k}}{\psi_{k}}} \leq \eps(\secparam)$, for every $k \in \{0,1\}^{\secparam}$ and $\eps(\cdot)$ is a negligible function. \noindent Let $\ket{\psi_k} = \sum_{x \in \{0,1\}^{d}} \alpha_{k,x} \ket{x}\ket{\psi_{k,x}}$ where $\alpha_{k,x}$ are nonnegative real numbers. We show the following: 
% \begin{equation}
% \label{eqn:prfs:stategen}
% \TraceDist{F_{\secparam}(k,x)}{\ketbra{\psi_{k,x}}{\psi_{k,x}}} \leq \eps'(\secparam),
% \end{equation}
% for some negligible function $\eps'(\cdot)$.
% \par We define a QPT algorithm $\widetilde{F}_{\secparam}(\cdot,\cdot)$ as follows: it takes as input $(\ket{\psi_k}^{\otimes 2^{d} \secparam},x)$, executes $F_{\secparam}(k,x)$ except that the step $\rho_k \leftarrow G_{\secparam}(k)$ is replaced with $\rho_k \leftarrow \ketbra{\psi_k}{\psi_k}$, in all of the $2^d \secparam$ executions. Consider the following two claims. 

% \begin{claim}
% \label{clm:stgen:close:proof}
% For all $k,x$ we have $\TraceDist{\widetilde{F}_{\secparam}\left( \ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{F_{\secparam}(k,x)} \leq 2^d \secparam\cdot \eps(\secparam)$.
% \end{claim}
% \begin{proof}
% From the monotonicity property of trace distance $(\star)$ and from the fact that $\TraceDist{\sigma_1^{\otimes L}}{\sigma_2^{\otimes L}} \leq L \cdot \TraceDist{\sigma_1}{\sigma_2}$ for any two mixed states $\sigma_1,\sigma_2$ and $L \in \mathbb{N}$ ($\star \star$), we have the following:

% \begin{align*}
% \TraceDist{\widetilde{F}_{\secparam}\left( \ketbra{\psi_k}{\psi_k}^{\otimes 2^{d}  \secparam},x \right)}{F_{\secparam}(k,x)}
% & \leq  \TraceDist{\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam}}{G_{\secparam}(k)^{\otimes 2^d \secparam}} &  (\star) \\
% & \leq  2^d \secparam \cdot \TraceDist{\ketbra{\psi_k}{\psi_k}}{G_{\secparam}(k)} & (\star \star) \\
% & \leq   2^d \secparam \cdot \varepsilon(\secparam)~. & 
% \end{align*}
% %$$\TraceDist{\widetilde{F}_{\secparam}\left( \ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{F_{\secparam}(k,x)} \leq \TraceDist{G_{\secparam}(k)}{\ketbra{\psi_k}{\psi_k}} \leq  \varepsilon(\secparam)$$
% Since $2^d$ is a polynomial in $\lambda$, this quantity is still negligible.
% \end{proof}

% \begin{claim}
% \label{clm:prfs:closetopure}
% For all $x \in \{0,1\}^d$, we have that \[
% \E_{k \leftarrow \{0,1\}^\lambda} \TraceDist{\widetilde{F}_{\secparam} \left( \ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{\ketbra{\psi_{k,x}}{\psi_{k,x}}} \leq \nu(\secparam)
% \]
% for some negligible function $\nu(\secparam)$.
% \end{claim}
% \begin{proof}
% Fix $k, x$. Observe that %$\widetilde{F}_{\secparam}\left(\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)$ is of the form: 
% \[
%     \widetilde{F}_{\secparam}\left(\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right) = (1-r_{k,x}) \ketbra{\psi_{k,x}}{\psi_{k,x}} + r_{k,x} \ketbra{\bot}{\bot}
% \]
% where $r_{k,x}$ is the probability that the measurement outcomes in all the $2^d \secparam$ repetitions is different from $x$ (i.e., the output of $\widetilde{F}_\lambda$ is $\ket{\bot}$). Since $\widetilde{F} = \{\widetilde{F}_\lambda\}_\secparam$ is a QPT algorithm, by the pseudorandomness property of $G$ we have that 
% \[
%     \left | \E_{k \leftarrow \{0,1\}^\lambda} r_{k,x} - \Pr_{\ket{\vartheta} \leftarrow \Haar_{d+n}} \left[  \widetilde{F}_{\secparam}\left(\ketbra{\vartheta}{\vartheta}^{\otimes 2^d \secparam},x \right) = \bot \right ] \right|
% \]
% is negligible. Thus to prove the Claim, it suffices to argue that the probability $\widetilde{F}_\lambda$ on input $(\ket{\vartheta}^{\otimes 2^d \secparam},x)$ outputs $\ket{\bot}$ for Haar-random $\ket{\vartheta}$ is negligible. 

% Define $p_{x}(\ket{\vartheta})$ to be the probability of obtaining outcome $x$ when measuring the first $d$ qubits of a state $\ket{\vartheta}$. We say that $\ket{\vartheta}$ is \emph{bad} if $p_x(\ket{\vartheta}) \leq 2^{-d}/2$ (and it is \emph{good} otherwise).  \Cref{lem:haar-prefix} implies that $\Pr_{\ket{\vartheta} \leftarrow \Haar_{d+n}} \left [ \text{$\ket{\vartheta}$ bad} \right ]$ is negligible in $\lambda$. Conditioned on $\ket{\vartheta}$ being good, the probability that $\widetilde{F}_\lambda$ on input $(\ket{\vartheta}^{\otimes 2^d \lambda},x)$ outputs $\ket{\bot}$ is going to be at most $(1 - 2^{-d-1})^{2^d \secparam} \leq e^{-\Omega(\lambda)}$ which is negligible. Thus
% \begin{align*}
% &\Pr_{\ket{\vartheta} \leftarrow \Haar_{d+n}} \left[  \widetilde{F}_{\secparam}\left(\ketbra{\vartheta}{\vartheta}^{\otimes 2^d \secparam},x \right) = \bot \right ] 
% \\
% & \qquad \qquad \qquad \leq \Pr_{\ket{\vartheta} \leftarrow \Haar_{d+n}} \left [ \text{$\ket{\vartheta}$ bad} \right ]  + \Pr_{\ket{\vartheta} \leftarrow \Haar_{d+n}} \left[  \widetilde{F}_{\secparam}\left(\ketbra{\vartheta}{\vartheta}^{\otimes 2^d \secparam},x \right) = \bot \Big | \text{$\ket{\vartheta}$ good} \right ]
% \end{align*}
% which is negligible, as desired.


% %Define $p_{k,x}$ to be the probability of obtaining outcome $x$ when measuring the first $d$ qubits of $\ket{\psi_k}$. By \Cref{lem:prs-prefix-prob}, the quantity $p_{k,x}$ is less than $2^{-d}/2$ with negligible probability over the choice of $k \leftarrow \{0,1\}^\lambda$. \note{HY: need to turn this into a high probability statement.} \pnote{it might be an overkill to apply Lemma 6 here (we only need Lemma 14). Here is how to think about this: if the states were Haar random then the probability that all the measurement outcomes fail is negligibly close to $\nu(\secparam)$ and so if we are dealing with $\ket{\psi_{k}}$, the probability of failure is also negligibly close to $\nu(\secparam)$ -- otherwise there is an efficient distinguisher which can distinguish $\ket{\psi_k}$ versus Haar random since we can test whether the experiment failed or not. The rest of the proof is the same.. I had this (ind. of Haar random) explicitly written when this was part of the QOTP construction and since I had to rewrite the proof all over again, this got lost.} \note{HY: good point! that's a much easier argument. I can try to add that in...} Thus, $\nu(\secparam) = (1-2^{-d})^{2^d \secparam} \leq e^{- \secparam}$ \note{HY: the probability of $x$ is not exactly $2^{-d}$. need to approx.}, which is a negligible function in $\secparam$. Thus,
% % \begin{eqnarray*}
% % \TraceDist{\widetilde{F}_{\secparam}\left(\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{\ketbra{\psi_{k,x}}{\psi_{k,x}}} & \leq &  (1-\nu(\secparam)) \cdot \TraceDist{\ketbra{\psi_{k,x}}{\psi_{k,x}}}{\ketbra{\psi_{k,x}}{\psi_{k,x}}}\\
% % & & +\ \nu(\secparam) \cdot \TraceDist{\ketbra{0}{0}}{\ketbra{\psi_{k,x}}{\psi_{k,x}}} \\
% % & \leq & \nu(\secparam)
% % \end{eqnarray*}


% \end{proof}

% \noindent Applying triangle inequality to the above two claims we have the following: 
% \begin{eqnarray*}
% \TraceDist{\widetilde{F}_{\secparam}\left(\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{\ketbra{\psi_{k,x}}{\psi_{k,x}}} & \leq & \TraceDist{\widetilde{F}_{\secparam}\left(\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{F_{\secparam}(k,x)}\\
% & & +\ \TraceDist{\widetilde{F}_{\secparam}\left(\ketbra{\psi_k}{\psi_k}^{\otimes 2^d \secparam},x \right)}{\ketbra{\psi_{k,x}}{\psi_{k,x}}} \\
% & \leq & 2^d \secparam \cdot \eps(\secparam) + \nu(\secparam) 
% \end{eqnarray*}
% Setting $\eps'=2^d \secparam \cdot \eps(\secparam) + \nu(\secparam)$ and observing that $\eps'(\secparam)$ is a negligible function,~\Cref{eqn:prfs:stategen} follows. 

%\paragraph{Pseudorandomness.}

